Evaluation of RAG Metrics for Question Answering in the Telecom Domain

Retrieval Augmented Generation (RAG) is widely used to enable Large Language Models (LLMs) perform Question Answering (QA) tasks in various domains. However, RAG based on open-source LLM for specialized domains has challenges of evaluating generated responses. A popular framework in the literature is the RAG Assessment (RAGAS), a publicly available library which uses LLMs for evaluation. One disadvantage of RAGAS is the lack of details of derivation of numerical value of the evaluation metrics. One of the outcomes of this work is a modified version of this package for few metrics (faithfulness, context relevance, answer relevance, answer correctness, answer similarity and factual correctness) through which we provide the intermediate outputs of the prompts by using any LLMs. Next, we analyse the expert evaluations of the output of the modified RAGAS package and observe the challenges of using it in the telecom domain. We also study the effect of the metrics under correct vs. wrong retrieval and observe that few of the metrics have higher values for correct retrieval. We also study for differences in metrics between base embeddings and those domain adapted via pre-training and fine-tuning. Finally, we comment on the suitability and challenges of using these metrics for in-the-wild telecom QA task.

==> duplicate_results_table_v2.tex <==
\begin{table*}
\centering
\scalebox{0.68}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{RAG LLM} & \textbf{RAGAS LLM} & \textbf{Embedding} & \textbf{Retr. Corr.} & \textbf{$FaiFul$}              & \textbf{$AnsRel$}            & \textbf{$ConRel$} & \textbf{$AnsSim$} & \textbf{$AnsCor$} & \textbf{Questions} & \textbf{$FacCor$}                      \\ \hline
Mistral          & Mistral            & BGE BASE           & Yes                  & 0.91(0.19)                         & 0.78(0.09)                      & 0.29(0.28)            & 0.73(0.1)                & 0.76(0.22)          & 502                & 0.77(0.29)                                  \\ \cline{4-11}
                 &                    &                    & No                   & 0.71(0.35)                         & 0.74(0.11)                      & 0.16(0.26)            & 0.61(0.09)               & 0.33(0.27)          & 213                & 0.24(0.34)                                  \\ \hline
Mistral          & Mistral            & BGE FT PT          & Yes                  & 0.91(0.19)                         & 0.55(0.12)                      & 0.28(0.28)            & 0.57(0.15)               & 0.71(0.23)          & 526                & 0.76(0.3)                                   \\ \cline{4-11}
                 &                    &                    & No                   & 0.78(0.31)                         & 0.5(0.13)                       & 0.19(0.27)            & 0.41(0.18)               & 0.3(0.29)           & 189                & 0.26(0.35)                                  \\ \hline
Mistral          & Mistral-IFT        & BGE FT PT          & Yes                  & 0.89(0.26)                         & \multicolumn{1}{l|}{0.36(0.12)} & 0.29(0.28)            & 0.84(0.22)               & 0.82(0.27)          & 526                & \textbf{0.82(0.31)} \\ \cline{4-11}
                 &                    &                    & No                   & 0.68(0.4)                          & \multicolumn{1}{l|}{0.36(0.11)} & 0.19(0.28)            & 0.57(0.26)               & 0.43(0.34)          & 189                & 0.38(0.39)          \\ \hline
Mistral          & Mistral            & LLM                & Yes                  & 0.91(0.18) & \textbf{0.9(0.04)}              & \textbf{0.3(0.29)}    & \textbf{0.88(0.05)}      & 0.79(0.22)          & 493                & 0.77(0.29)          \\ \cline{4-11}
                 &                    &                    & No                   & 0.71(0.35) & 0.88(0.04)                      & 0.15(0.25)            & 0.82(0.04)               & 0.37(0.25)          & 222                & 0.22(0.33)          \\ \hline
Mistral          & Mistral            & LLM PT FT          & Yes                  & 0.91(0.19) & 0.7(0.09)                       & 0.29(0.28)            & 0.68(0.11)               & 0.75(0.23)          & 515                & 0.77(0.29)          \\ \cline{4-11}
                 &                    &                    & No                   & 0.77(0.31) & 0.65(0.09)                      & 0.19(0.28)            & 0.53(0.11)               & 0.32(0.28)          & 200                & 0.24(0.35)          \\ \hline
Mistral          & Mistral-IFT        & LLM PT FT          & Yes                  & 0.88(0.26) & 0.48(0.09)                      & 0.29(0.28)            & 0.88(0.17)               & \textbf{0.83(0.27)} & 515                & 0.81(0.31)          \\ \cline{4-11}
                 &                    &                    & No                   & 0.64(0.42) & 0.48(0.09)                      & 0.19(0.28)            & 0.64(0.21)               & 0.43(0.33)          & 200                & 0.36(0.39)          \\ \hline
GPT3.5           & GPT 3.5            & BGE FT PT          & Yes                  & \textbf{0.94(0.17)}                & 0.88(0.05)                      & 0.18(0.2)             & 0.87(0.05)               & 0.8(0.21)           & 526                & 0.78(0.26)                                  \\ \cline{4-11}
                 &                    &                    & No                   & 0.68(0.42)                         & 0.83(0.08)                      & 0.13(0.22)            & 0.8(0.06)                & 0.39(0.3)           & 189                & 0.26(0.37)                                  \\ \hline
\end{tabular}
}
\caption{RAGAS Metrics for our dataset with $k=1$ retrieved contexts being passed. Numbers are mean(s.d.). BGE BASE is the publicly available emebdding for \textit{bge-large-en}, BGE PT FT is the pre-trained finetuned model for the same. Similar notation is followed for \textit{llm-embedder}. Mistral-IFT is the instruction finetuned mistral model. GPT3.5 is the ada-002 embeddings.\label{tab:ragas_metrics_v2_xx}}
\end{table*}

==> results_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
\scalebox{0.72}{
\begin{tabular}{|ll|l|l|l|lllll|l|}
\hline
\multicolumn{2}{|c|}{LLM Used}                                              & Embedding                                                                                                           & Type of data & Retrieval & \multicolumn{5}{c|}{RAGAS Metrics: Mean (SD)}                                                                                                              &            \\ \hline
\multicolumn{1}{|l|}{Generator}                 & RAGAS                     &                                                                                                                     &              &           & \multicolumn{1}{l|}{$FaiFul$} & \multicolumn{1}{l|}{$AnsRel$}    & \multicolumn{1}{l|}{$ConRel$} & \multicolumn{1}{l|}{$AnsSim$}    & $AnsCor$ & \#Qs Retr. \\ \hline
\multicolumn{1}{|l|}{\multirow{24}{*}{Mistral}} & \multirow{24}{*}{Mistral} & \multirow{8}{*}{GTE}                                                                                                & GT Answer    & NA        & \multicolumn{1}{l|}{0.92 (0.24)}  & \multicolumn{1}{l|}{0.25(0.16)} & \multicolumn{1}{l|}{0.23(0.35)}  & \multicolumn{1}{l|}{1(0.0)}     & 1(0.0)          & 715        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & GT Context   & NA        & \multicolumn{1}{l|}{0.91(0.18)}   & \multicolumn{1}{l|}{0.63(0.16)} & \multicolumn{1}{l|}{0.23(0.24)}  & \multicolumn{1}{l|}{0.54(0.18)} & 0.69(0.24)      & 715        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-1        & Yes       & \multicolumn{1}{l|}{0.91(0.18)}   & \multicolumn{1}{l|}{0.65(0.15)} & \multicolumn{1}{l|}{0.28(0.28)}  & \multicolumn{1}{l|}{0.54(0.18)} & 0.7(0.24)       & 567        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-1        & No        & \multicolumn{1}{l|}{0.85(0.25)}   & \multicolumn{1}{l|}{0.59(0.15)} & \multicolumn{1}{l|}{0.22(0.27)}  & \multicolumn{1}{l|}{0.36(0.18)} & 0.37(0.31)      & 148        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-3        & Yes       & \multicolumn{1}{l|}{0.9(0.19)}    & \multicolumn{1}{l|}{0.64(0.15)} & \multicolumn{1}{l|}{0.13(0.15)}  & \multicolumn{1}{l|}{0.53(0.18)} & 0.68(0.24)      & 629        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-3        & No        & \multicolumn{1}{l|}{0.84(0.28)}   & \multicolumn{1}{l|}{0.57(0.16)} & \multicolumn{1}{l|}{0.11(0.15)}  & \multicolumn{1}{l|}{0.32(0.2)}  & 0.33(0.33)      & 86         \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-5        & Yes       & \multicolumn{1}{l|}{0.89(0.21)}   & \multicolumn{1}{l|}{0.63(0.21)} & \multicolumn{1}{l|}{0.08(0.21)}  & \multicolumn{1}{l|}{0.51(0.21)} & 0.66(0.21)      & 653        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-5        & No        & \multicolumn{1}{l|}{0.79(0.3)}    & \multicolumn{1}{l|}{0.57(0.15)} & \multicolumn{1}{l|}{0.09(0.14)}  & \multicolumn{1}{l|}{0.3(0.19)}  & 0.26(0.3)       & 62         \\ \cline{3-11} 
\multicolumn{1}{|l|}{}                          &                           & \multirow{8}{*}{GPT Embeddings}                                                                                     & GT Answer    & NA        & \multicolumn{1}{l|}{0.92 (0.24)}  & \multicolumn{1}{l|}{0.76(0.05)} & \multicolumn{1}{l|}{0.23(0.35)}  & \multicolumn{1}{l|}{1(0.0)}     & 1(0.0)          & 715        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & GT Context   & NA        & \multicolumn{1}{l|}{0.91(0.18)}   & \multicolumn{1}{l|}{0.64(0.13)} & \multicolumn{1}{l|}{0.23(0.24)}  & \multicolumn{1}{l|}{0.59(0.16)} & 0.74(0.3)       & 715        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-1        & Yes       & \multicolumn{1}{l|}{0.91(0.19)}   & \multicolumn{1}{l|}{0.65(0.13)} & \multicolumn{1}{l|}{0.29(0.28)}  & \multicolumn{1}{l|}{0.58(0.16)} & 0.71(0.24)      & 516        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-1        & No        & \multicolumn{1}{l|}{0.81(0.27)}   & \multicolumn{1}{l|}{0.59(0.14)} & \multicolumn{1}{l|}{0.19(0.27)}  & \multicolumn{1}{l|}{0.43(0.16)} & 0.33(0.3)       & 199        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-3        & Yes       & \multicolumn{1}{l|}{0.89(0.2)}    & \multicolumn{1}{l|}{0.64(0.13)} & \multicolumn{1}{l|}{0.11(0.14)}  & \multicolumn{1}{l|}{0.58(0.16)} & 0.69(0.25)      & 614        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-3        & No        & \multicolumn{1}{l|}{0.87(0.23)}   & \multicolumn{1}{l|}{0.59(0.15)} & \multicolumn{1}{l|}{0.09(0.15)}  & \multicolumn{1}{l|}{0.44(0.16)} & 0.34(0.29)      & 101        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-5        & Yes       & \multicolumn{1}{l|}{0.9(0.19)}    & \multicolumn{1}{l|}{0.64(0.13)} & \multicolumn{1}{l|}{0.07(0.1)}   & \multicolumn{1}{l|}{0.57(0.16)} & 0.67(0.25)      & 645        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-5        & No        & \multicolumn{1}{l|}{0.79(0.31)}   & \multicolumn{1}{l|}{0.59(0.15)} & \multicolumn{1}{l|}{0.06(0.08)}  & \multicolumn{1}{l|}{0.41(0.15)} & 0.29(0.29)      & 70         \\ \cline{3-11} 
\multicolumn{1}{|l|}{}                          &                           & \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}bge\_large\_en\\ pretrained,\\ finetuned\end{tabular}}                   & GT Answer    & NA        & \multicolumn{1}{l|}{0.92 (0.24)}  & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{0.23(0.35)}  & \multicolumn{1}{l|}{1(0.0)}     & 1(0.0)          & 715        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & GT Context   & NA        & \multicolumn{1}{l|}{0.91(0.18)}   & \multicolumn{1}{l|}{0.54(0.13)} & \multicolumn{1}{l|}{0.23(0.24)}  & \multicolumn{1}{l|}{0.57(0.15)} & 0.7(0.24)       & 715        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-1        & Yes       & \multicolumn{1}{l|}{0.91(0.19)}   & \multicolumn{1}{l|}{0.55(0.12)} & \multicolumn{1}{l|}{0.28(0.28)}  & \multicolumn{1}{l|}{0.57(0.15)} & 0.71(0.23)      & 526        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-1        & No        & \multicolumn{1}{l|}{0.78(0.31)}   & \multicolumn{1}{l|}{0.5(0.13)}  & \multicolumn{1}{l|}{0.19(0.27)}  & \multicolumn{1}{l|}{0.41(0.18)} & 0.3(0.29)       & 189        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-3        & Yes       & \multicolumn{1}{l|}{0.89(0.2)}    & \multicolumn{1}{l|}{0.54(0.12)} & \multicolumn{1}{l|}{0.11(0.14)}  & \multicolumn{1}{l|}{0.57(0.15)} & 0.68(0.25)      & 632        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-3        & No        & \multicolumn{1}{l|}{0.85(0.26)}   & \multicolumn{1}{l|}{0.48(0.13)} & \multicolumn{1}{l|}{0.14(0.19)}  & \multicolumn{1}{l|}{0.45(0.17)} & 0.35(0.32)      & 83         \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-5        & Yes       & \multicolumn{1}{l|}{0.89(0.2)}    & \multicolumn{1}{l|}{0.54(0.13)} & \multicolumn{1}{l|}{0.07(0.09)}  & \multicolumn{1}{l|}{0.56(0.15)} & 0.67(0.25)      & 665        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-5        & No        & \multicolumn{1}{l|}{0.8(0.25)}    & \multicolumn{1}{l|}{0.46(0.12)} & \multicolumn{1}{l|}{0.1(0.16)}   & \multicolumn{1}{l|}{0.43(0.18)} & 0.33(0.32)      & 50         \\ \hline
\multicolumn{1}{|l|}{\multirow{8}{*}{GPT3.5}}   & \multirow{8}{*}{GPT3.5}   & \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Best Embedding\\ bge\_large\_en\\ pretrained,\\ finetuned)\end{tabular}} & GT Answer    & NA        & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}           &                 &            \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & GT Context   & NA        & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}           &                 &            \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-1        & Yes       & \multicolumn{1}{l|}{0.94(0.17)}   & \multicolumn{1}{l|}{0.88(0.05)} & \multicolumn{1}{l|}{0.18(0.2)}   & \multicolumn{1}{l|}{0.87(0.05)} & 0.8(0.21)       & 526        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-1        & No        & \multicolumn{1}{l|}{0.68(0.42)}   & \multicolumn{1}{l|}{0.83(0.08)} & \multicolumn{1}{l|}{0.13(0.22)}  & \multicolumn{1}{l|}{0.8(0.06)}  & 0.39(0.3)       & 189        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-3        & Yes       & \multicolumn{1}{l|}{0.93(0.18)}   & \multicolumn{1}{l|}{0.88(0.05)} & \multicolumn{1}{l|}{0.06(0.07)}  & \multicolumn{1}{l|}{0.87(0.05)} & 0.77(0.24)      & 632        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-3        & No        & \multicolumn{1}{l|}{0.76(0.39)}   & \multicolumn{1}{l|}{0.85(0.08)} & \multicolumn{1}{l|}{0.07(0.17)}  & \multicolumn{1}{l|}{0.8(0.07)}  & 0.42(0.31)      & 83         \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-5        & Yes       & \multicolumn{1}{l|}{0.83(0.32)}   & \multicolumn{1}{l|}{0.86(0.08)} & \multicolumn{1}{l|}{0.03(0.06)}  & \multicolumn{1}{l|}{0.85(0.08)} & 0.72(0.27)      & 665        \\ \cline{4-11} 
\multicolumn{1}{|l|}{}                          &                           &                                                                                                                     & Top-5        & No        & \multicolumn{1}{l|}{0.75(0.37)}   & \multicolumn{1}{l|}{0.85(0.06)} & \multicolumn{1}{l|}{0.04(0.07)}  & \multicolumn{1}{l|}{0.8(0.06)}  & 0.38(0.31)      & 50         \\ \hline
\end{tabular}
}
\caption{Results for RAG Metrics}
\label{tab:results}
\end{table*}
